Data-Driven Performance Guarantees for Parametric Optimization Problems

We propose a data-driven method to establish probabilistic performance guarantees for parametric optimization problems solved via iterative algorithms. Our approach addresses two key challenges: providing convergence guarantees to characterize the worst-case number of iterations required to achieve a predefined tolerance, and upper bounding a performance metric after a fixed number of iterations. These guarantees are particularly useful for online optimization problems with limited computational time, where existing performance guarantees are often unavailable or unduly conservative. We formulate the convergence analysis problem as a scenario optimization program based on a finite set of sampled parameter instances. Leveraging tools from scenario optimization theory enables us to derive probabilistic guarantees on the number of iterations needed to meet a given tolerance level. Using recent advancements in scenario optimization, we further introduce a relaxation approach to trade the number of iterations against the risk of violating convergence criteria thresholds. Additionally, we analyze the trade-off between solution accuracy and time efficiency for fixed-iteration optimization problems by casting them into scenario optimization programs. Numerical simulations demonstrate the efficacy of our approach in providing reliable probabilistic convergence guarantees and evaluating the trade-off between solution accuracy and computational cost.

==> old_section_2.tex <==
% Previous version of 2.B & 2.C
\subsection{Scenario optimization}
% Define the necessary component in scenario approach formulation
Before proceeding, we first introduce some concepts in scenario optimization and discuss their relevance to our problem.

\begin{definition}[Support constraint, {\protect{\cite[Definition 2]{GarattiCampi2022}}}] \label{support_constraint} A constraint \( y \geq n_i \) of the scenario optimization problem \eqref{n scenario} is called a \emph{support constraint} if its removal (while all other constraints are maintained) changes the solution \( n_N^* \). 
%The \emph{complexity} of the scenario optimization problem (1) is the number of its support constraints. \hfill \(\square\)
\end{definition}
The concept of \emph{support constraint} plays a crucial role in scenario optimization. Most scenario approach bounds rely on the \emph{non-degeneracy} assumption, which requires the optimal solution of the scenario optimization problem to remain unchanged after removing all the constraints that are not support constraints \cite[Definition 3]{GarattiCampi2022}. 

However, the optimization problem \eqref{n scenario} is degenerate. This is because the scenario constraints generated by the samples are discrete and finite, making it highly probable that some constraints coincide, i.e., \( n_i = n_j \) for some \( i \neq j \). When multiple active constraints coincide then by convention \emph{none} are considered support constraints, since removing any one of them in isolation does not alter the optimal solution of problem \eqref{n scenario}, which involves only one decision variable. Nevertheless, if all non-support constraints are removed, the optimal solution will change, indicating that problem \eqref{n scenario} is not non-degenerate. Therefore, the convex scenario approach \cite{GarattiCampi2022, Marco_CDC_2020} does not apply to our problem \eqref{n scenario} and its relaxed version in the late section. Recent advancements in the scenario approach \cite{non-convex_scenario_optimization2024} have eliminated the need for the non-degeneracy assumption, extending the applicability of the scenario approach to problems like ours.
%PG : paragraph above could be shorter probably.

The problem \eqref{n scenario} models a decision-making process. This process can be understood as a mapping \( M_N : \Delta^N \to \mathbb{R} \), where \( M_N \) maps a collection of \( N \) samples from the sample space \(\Delta\) to an optimal decision \(y^*_N = n^*_N \in \mathbb{R} \). Since the decision $n^*_N$ returned by $M_N$ depends on the samples $x_1, \ldots, x_N$, we explicitly highlight this dependency by using the notation \( M_N(x_1, \ldots, x_N) \). The following property is fundamental to our study. 
%non-convex scenario optimization. 

\begin{definition}[Consistency property, {\protect{\cite[Property 1]{non-convex_scenario_optimization2024}}}]\label{consistency_property}
For any integers \( N \geq 0 \) and \( M > 0 \) and for any choice of \(x_1, \ldots, x_N\) and \(x_{N+1}, \ldots, x_{N+M}\), the following three conditions hold:
\begin{enumerate}
    \item[(i)] If \(x_{i_1}, \ldots, x_{i_N}\) is a permutation of \(x_1, \ldots, x_N\), then it holds that $ M_N(x_1, \ldots, x_N) = M_N(x_{i_1}, \ldots, x_{i_N});$
    \item[(ii)] If \(y^*_N \in Y_{x_{N+i}}\) for all \(i = 1, \ldots, M\), then it holds that $y^*_{N+M} = M_{N+M}(x_1, \ldots, x_{N+M}) = M_N(x_1, \ldots, x_N) = y^*_N;$
    \item[(iii)] If \(y^*_N \notin Y_{x_{N+i}}\) for one or more \(i \in \{1, \ldots, M\}\), then it holds that $y^*_{N+M} = M_{N+M}(x_1, \ldots, x_{N+M}) \neq M_N(x_1, \ldots, x_N) = y^*_N.$
\end{enumerate}
\end{definition}

Here, \( Y_{x_i} \) represents the feasible domain defined by the scenario constraint corresponding to the \( i \)th sample \( x_i \). 
%PJG: I think this notation should be introduced either above or within Definition II.2
Condition (i) is referred to as \emph{permutation invariance}, meaning that the decision of the map \( M_N \) remains unchanged regardless of the order of scenarios. Condition (ii) is the \emph{confirmation under appropriateness}, which ensures that the  decision remains the same when additional scenarios are introduced, provided the previous decision already satisfies the constraints imposed by these new scenarios. Condition (iii) is the \emph{responsiveness to inappropriateness}, which requires that the decision-making process $M_N$ reacts when additional scenarios are added for which the previous decision does not meet the constraints induced by these new scenarios.

\subsection{Probabilistic convergence guarantees}\label{section:robust convergence guarantee}
% PAC guarantee for the convergence problem
In the previous section, we concluded that problem \eqref{n scenario} is degenerate, making convex scenario optimization inapplicable. This leaves us with non-convex scenario optimization as the alternative. Now, we must verify that the mapping \( M_N \) defined in \eqref{n scenario} satisfies the consistency property to apply non-convex scenario optimization.

\begin{lemma}\label{consistency_proof}
    Consider the scenario optimization problem \eqref{n scenario}, the mapping \( M_N \) satisfies the consistency property.
\end{lemma}

\textit{Proof.} Condition (i) holds because the solution to \eqref{n scenario} is independent of the order of constraints. Now, examine conditions (ii) and (iii). Suppose $M$ new constraints \( y \geq n_{N+i} \) for \( i = 1, \ldots, M \)  are added to the original constraint set \( y \geq n_i \) for \( i = 1, \ldots, N \). If \( n^*_N \geq n_{N+i} \) for all \( i = 1, \ldots, M \), then \( n^*_N \) remains feasible in the expanded problem with \( N+M \) constraints. Since the optimal solution does not change, we have \( n^*_{N+M} = n^*_N \), confirming condition (ii). Conversely, if \( n^*_N < n_{N+i} \) for some \( i \), then \( n^*_N \) is no longer feasible in the new problem. As a result, the optimal solution must change to satisfy the additional constraints, meaning \( n^*_{N+M} \neq n^*_N \), which establishes condition (iii).  \hfill \(\square\)

% Define the definition of violation

Thus, the non-convex scenario optimization approach from \cite{non-convex_scenario_optimization2024} can be applied to establish a probabilistic generalization guarantee for problem \eqref{n scenario}. We define \emph{risk} \( V(n^*_N) = \mathbb{P}\{x \in \Delta : n_x > n^*_N \} \), which quantifies the probability level of  violating the convergence condition for an unseen sample $\delta$. This probability cannot be computed, as its calculation requires full knowledge of \(\mathbb{P}\), which is either unavailable or only partially known. A key advantage of the scenario approach is that it can provide guarantees on the risk \(V(n_N^*)\) without requiring additional samples beyond those used in optimization. It can provide a probabilistically approximately correct (PAC) statement as follows,
\begin{equation}\label{PAC_statement}
\mathbb{P}^N \{ V(n_N^*) < \epsilon \} \geq 1- \beta,
\end{equation}
where $\epsilon$ is an upper bound on the true violation probability $V(n_N^*)$ with confidence at least $1-\beta$. Note that the value of $n^*_N$ is random and depends on the set of samples $(x_1, \ldots, x_N) \in \Delta^N$, with a distribution of $\mathbb{P}^N$, that is the reason of having the second probabilistic bound $1-\beta$. 

Given a user-chosen confidence lever $\beta$, consider the polynomial equation \cite{non-convex_scenario_optimization2024} in the $t$ variable, for any $l = 0, 1, \ldots, N-1$,
\begin{equation}\label{compute_t}
\frac{\beta}{N} \sum_{m=l}^{N-1} \binom{m}{l} t^{m-l} - \binom{N}{l} t^{N-l} = 0,
\end{equation}
where $N$ is the number of samples. Equation \eqref{compute_t} has one and only solution \( t(l) \) within the interval \((0, 1)\). \( \epsilon(l) \) is then given by:
\begin{equation}\label{compute_epsilon}
\begin{split}
    \epsilon(l) := \left\{
\begin{array}{ll}
      1 - t(l), & \text{if } l = 0, 1, \ldots, N-1, \\
      1, & \text{if } l = N.
\end{array}
\right. \\
\end{split}
\end{equation}

\begin{theorem}\label{theorem 1} Consider the scenario optimization problem \eqref{n scenario}. For any $\mathbb{P},$ it holds that
\begin{equation}
\mathbb{P}^N \{ V(n_N^*) < \epsilon(s^*_N) \} \geq 1- \beta,
\end{equation}
where $\epsilon$ can be computed with equations \eqref{compute_t} and \eqref{compute_epsilon}, with complexity $s_N^* = 1$.
\end{theorem}

\textit{Proof.} In Lemma \ref{consistency_proof}, we have proved the consistency property of the map $M_N$ defined by problem \eqref{n scenario}. Therefore, we can apply \cite[Theorem 6]{non-convex_scenario_optimization2024} to compute the value of $\epsilon$ in equation \eqref{PAC_statement}. Given that problem \eqref{n scenario} is a convex scenario optimization problem with only a single decision variable, the minimum number of scenario constraints required to determine the optimal solution \(n^*_N\) is one. Consequently, its complexity $s_N^* = 1$, meaning that just one critical scenario constraint is sufficient to fully characterize the optimal solution. \hfill \(\square\)

\textbf{Remark 1.} Equation \eqref{compute_t} and \eqref{compute_epsilon} correspond to a posteriori probabilistic bounds that the complexity is decided after solving the scenario optimization problem. Here, we used them in a-priori manner and the reason is for better flow of the paper, as we will introduce constraint relaxation to problem \eqref{n scenario} and existing a-priori probabilistic bounds are not applicable for the relaxed problem. Since the current problem can be solved in a-priori manner, and problem \eqref{n scenario} is convex, the confidence $\beta$ and violation probability $\epsilon$ follow a binomial tail distribution that $\beta := \sum_{i=0}^{d-1} \binom{N}{i} \epsilon^i (1 - \epsilon)^{N-i}$ \cite{campi2008exact, Kostas_2015}, the inverse computation for $\epsilon$ will give a tight estimate for $\epsilon$. However, as mentioned, previously it is not applicable for the later relaxation analysis. 

Although problem \eqref{n scenario} is degenerate, its convexity allows us to apply the bounds from \cite[Theorem 1, 2]{Kostas_2015} to compute the value of \( \epsilon \) in equation \eqref{PAC_statement}.  Among these bounds, \cite[Theorem 3]{Kostas_2015} provides a tighter bound than the one obtained from solving equations \eqref{compute_t} and \eqref{compute_epsilon}, as it holds with equality for fully-supported problems \cite{campi2008exact}. However, we do not introduce \cite[Theorem 3]{Kostas_2015} in detail here because it does not apply to the constraint relaxation approach discussed in the next section. For consistency in the paper, we primarily present equations \eqref{compute_t} and \eqref{compute_epsilon}. Nevertheless, given our problem formulation, the bounds from \cite{campi2008exact} and \cite{Kostas_2015} can also be used to compute \( \epsilon \), providing an upper bound on the true violation probability \( V(n^*_N) \). In the numerical examples, we compute and compare all three bounds to evaluate their tightness.

\subsection{Relaxed convergence guarantees}
% Formulate the relaxed scenario optimization

% Describe the method of choosing the parameters

In the previous section, we analyzed problem \eqref{n scenario}, a robust scenario optimization problem. Here, we extend this framework to a relaxed scenario optimization problem to evaluate the trade-off between the number of iterations and the probability of convergence. This trade-off analysis is particularly valuable in online optimization settings, where there may not be sufficient time for problem \eqref{parametric_optimization_problem} to converge. Following this approach, users can determine appropriate iteration budgets that balance computational efficiency with satisfactory convergence performance in online optimization.

In this section, we consider the following PAC statement:  
\begin{equation}\label{relaxed_PAC statement}
    \mathbb{P}^N \{x_1, ..., x_N: \mathbb{P}(x \in \Delta: n_x  > n_a) \leq \epsilon_a\} \geq 1 - \beta,
\end{equation}  
where \( n_x  \) represents the number of iterations required for a new sample \( x \in \Delta \) of the problem parameter \( x \) in \eqref{parametric_optimization_problem} to achieve convergence. The quantity \( n_a \) denotes the iteration budget, while \( \epsilon_a \) is the upper bound of the probability of violation given \( n_a \). When \( n_a \) is large, most samples can converge within the allowed iterations, resulting in a small violation probability \( \epsilon_a \). The statement \eqref{relaxed_PAC statement} aims to address situations where the available iteration budget is insufficient to guarantee convergence. 

The trade-off problem can be formulated as a relaxed version of the robust scenario optimization problem \eqref{n scenario}:  
\begin{equation}\label{n_relaxed scenario optimization}
\begin{split}
    \min_{y, \, \xi_{N,i} \geq 0, \, i=1,\ldots,N} \quad & y + \rho \sum_{i=1}^N \xi_{N,i}\\
    \text{subject to:} \quad & y + \xi_{N,i} \geq n_i, \quad i = 1, \ldots, N,
\end{split}
\end{equation}  
where \( \xi_{N,i}, i = 1, \ldots, N \) are relaxation variables and weight $\rho > 0$. When \( \xi_{N,i} > 0 \), the original constraint \( y \geq n_i \) is relaxed to \( y + \xi_{N,i} \geq n_i \). The optimal solution $y_N^*$ is also denoted $n^*_N(\rho)$ to emphasize its connection with \( n^*_N \) in \eqref{n scenario}. Once problem \eqref{n_relaxed scenario optimization} is solved, the number of constraints that are violated (i.e., where \( \xi^*_{N,i} > 0 \)) is denoted \( q_N^* \). The objective function in \eqref{n_relaxed scenario optimization} is strictly convex in all optimization variables. Given the variables have no upper bound, the optimization problem \eqref{n_relaxed scenario optimization} always admits a \emph{unique} solution.

Since problem \eqref{n_relaxed scenario optimization} represents a decision-making process, we consider an augmented decision variable \( \tilde{y}_N^* = (y_N^*, q_N^*) \) \cite{non-convex_scenario_optimization2024}, which captures both the optimized solution and the number of relaxed constraints.  The mapping from the set of \( N \) independent samples \( \{x_1, \ldots, x_N\} \) to the augmented decision \( \tilde{y}_N^* \) is denoted \( M_N^{relax} \), where \( M_N^{relax} : \Delta^N \rightarrow \mathbb{R}^2 \). To establish a probabilistic guarantee, it is necessary to confirm that \( M_N^{relax} \) satisfies the consistency property.

\begin{lemma}\label{relaxed_consistency_proof}
    Consider the relaxed scenario optimization problem \eqref{n_relaxed scenario optimization}, the map \( M_N^{relax} \) satisfies the consistency property in Definition \ref{consistency_property}.
\end{lemma}

\textit{Proof.} Condition (i) holds because $y_N^*$ and $q_N^*$ are independent of the order of constraints, so is $\tilde{y}_N^*$. Now, examine conditions (ii) and (iii). Adding $M$ new scenarios $x_{N+1}, \ldots, x_{N+M}$ to the original samples $x_1, \ldots, x_N$ and assume that \( y_N^* \geq n_{N+i} \) for all \( i = 1, \ldots, M \). Consider problem \eqref{n_relaxed scenario optimization} with $N+M$ in place of $N$. Since \( y_N^* \geq n_{N+i} \) for all \( i = 1, \ldots, M \) meaning $ (y_N^*, \xi_{N,1}^*, \ldots, \xi_{N,N}^*, 0, \ldots, 0)$ is feasible for problem \eqref{n_relaxed scenario optimization} with $N+M$ scenarios. We claim that this is indeed the optimal solution, which can be shown by contradiction. If the optimal solution were different, and it is denoted \( (\bar{y}, \bar{\xi}_{N+M,i}) \) for \( i = 1, \dots, N+M \), then one of the following two cases must hold:

\begin{enumerate}
    \item[(a)] \( \bar{y} + \rho \sum_{i=1}^{N+M} \bar{\xi}_{N+M,i} < y^*_N + \rho \sum_{i=1}^{N} \xi_{N,i}^* \). This implies that \( \bar{y} + \rho \sum_{i=1}^{N} \bar{\xi}_{N+M,i} < y^*_N + \rho \sum_{i=1}^{N} \xi_{N,i}^*\) since the omitted terms \(\bar{\xi}_{N+M,i} \geq 0, \text{ for } i = N+1, \ldots, N+M\)). This means that in problem \eqref{n_relaxed scenario optimization}, the solution \( (\bar{y}, \bar{\xi}_{N+M,i}, i = 1, \dots, N) \) achieves a better objective value than the optimal solution \( (y_N^*, \xi^*_{N,i}, i = 1, \dots, N) \), leading to a contradiction.

    \item[(b)] \( \bar{y} + \rho \sum_{i=1}^{N+M} \bar{\xi}_{N+M,i} = y^*_N + \rho \sum_{i=1}^{N} \xi_{N,i}^*\) and $\bar{y} \neq y^*_N$. By omitting terms \(\bar{\xi}_{N+M,i} \geq 0, \text{ for } i = N+1, \ldots, N+M\)), we have \(\bar{y} + \rho \sum_{i=1}^{N} \bar{\xi}_{N+M,i} \leq y^*_N + \rho \sum_{i=1}^{N} \xi_{N,i}^*.\) If this inequality holds strictly, it would lead to a contradiction similar to case (a). On the other hand, if equality holds, it implies that problem \eqref{n_relaxed scenario optimization} with $N$ scenarios has multiple optimal solutions. However, since the problem is strictly convex, it must have a unique optimal solution, leading to a contradiction.
\end{enumerate}

Hence, we have proven that $(y_N^*, \xi_{N,1}^*, \ldots, \xi_{N,N}^*, 0, \ldots, 0)$ is the unique optimal solution for problem \eqref{n_relaxed scenario optimization} when extended to \( N+M \) constraints. Consequently, the decision returned by the mapping \( M_N^{\text{relax}} \) remains unchanged, i.e., $\tilde{y}_{N+M}^* = (y_{N+M}^*, q^*_{N+M}) = (y_{N}^*, q^*_{N}) = \tilde{y}_{N}^*$, which proves condition (ii) in the consistency property.

Now, suppose instead that \( y_N^* < n_{N+i} \) for some \( i \). If \( y_{N+M}^* = y_N^* \), then $ \xi_{N+M, i}^* = \xi_{N, i}^* \text{ for } i = 1, \ldots, N \text{ and } \xi_{N+M, N+i}^* > 0 \text{ for some } i$. As a result, $q_{N+M}^* > q_N^*,$ which implies that \(\tilde{y}_{N+M}^* \neq \tilde{y}_{N}^*\). Alternatively, if \(y_{N+M}^* \neq y_N^*\), it directly follows that \( \tilde{y}_{N+M}^* \neq \tilde{y}_N^* \). This proves condition (iii). \hfill \(\square\)

\begin{theorem} Consider the relaxed scenario optimization problem \eqref{n_relaxed scenario optimization}. For any $\mathbb{P},$ it holds that
\begin{equation}\label{relaxed_pac}
\mathbb{P}^N \{x_1, ..., x_N: V(n^*_N(\rho)) \leq \epsilon(s^*_N)\} \geq 1 - \beta,
\end{equation}
where $\epsilon_\rho$ can be computed with equations \eqref{compute_t} and \eqref{compute_epsilon}, with $s_N^* = 1 + q_N^*$.
\end{theorem}

\textit{Proof.} In Lemma \ref{consistency_proof}, we have proved the consistency property of the map $M_N^{relax}$. This allows us to apply \cite[Theorem 10]{non-convex_scenario_optimization2024} to compute \( \epsilon_\rho \) in equation \eqref{relaxed_pac}. In problem \eqref{n_relaxed scenario optimization}, the number of scenarios \(x_i\) for which \(\xi_i^* > 0\) (i.e., violated constraints) is combined with a minimal number of additional scenarios \(x_i\) that, together with the violated ones, fully determine \(y_N^*\) as the \(y\)-component of the solution. For our problem, since \(y\) is a scalar and the problem is convex, only \emph{one additional constraint} is sufficient to uniquely determine \(y\). Therefore, the total number of scenarios required to characterize the solution is \(s^*_N = 1 + q_N^*\), where \(q_N^*\). \hfill \(\square\)

The user-defined parameter $\rho$ sets a trade-off between minimizing the original cost function and penalizing the violation of constraints. To ensure an appropriate balance, we propose a systematic method for selecting the value of \(\rho\).

Problem \eqref{n_relaxed scenario optimization} can be formulated as an unconstrained optimization problem $\min_{y}\; f(y)$, where

\begin{equation}
    f(y) =  y + \rho \sum_{i=1}^N \max\{0, n_i - y\}. 
\end{equation}

The sub-gradient $\frac{df}{dy} = 1 + \rho \sum^N_{i=1} h_i(y)$, with  

\begin{equation}\label{define_h}
\begin{split}
    h_i(y) := \left\{
\begin{array}{ll}
      0, & \text{if } n_i < y, \\
      -1, & \text{if } n_i \geq y.
\end{array}
\right. \\
\end{split}
\end{equation}

At the optimal solution, the derivative of the cost function satisfies \(\frac{df}{dy}|_{n^*_N(\rho)} = 1 + \rho \sum^N_{i=1} h_i(n^*_N(\rho)) =  0\). Solving for \(\rho\), we obtain:
\[
\rho = \frac{-1}{\sum^N_{i=1} h_i(n^*_N(\rho))}.
\]
The denominator can be interpreted as \(-1\) times the number (or fraction) of constraints that we are willing to violate to reduce the optimal iteration number \(n^*_N(\rho)\). Since the fraction of constraints we targeted to violated can be pre-defined and is independent of the samples, we denote this quantity as $\hat{q}_N$. $\hat{q}_N$ is an approximation of the number of constraints we actually violated, which equals $q^*_N$, and we can use the parameter \(\rho = \frac{1}{\hat{q}_N}\) when solving problem \eqref{n_relaxed scenario optimization}.

% not paraphrased
\textbf{Remark 2.} Compare with \cite{sambharya_data-driven_2024}. From result perspective -- two main points, 1. Not able to estimate the convergence guarantee from an empirical estimate for the convergence guarantee. 2. Pre-define the iteration number and then compute the violation probability, while our method, predefined the number of samples we want to be relaxed, i.e., the empirical violation probability.

From the method perspective --- Their bound rooted from test bound theorem \cite{JMLR:v6:langford05a} that estimates true error from empirical error, it is a task of generalization only. Our method uses scenario optimization, learning the optimization variable $n^*_N$ and provide a generalization guarantee as well, doing the learning and generalization task simultaneously. 




==> redundant.tex <==
section 2 B - Kostas
Moreover, such an optimization problem belongs to the class of fully-supported programs \cite{modulating_robustness_2013}, which in turn implies that the right-hand side in 
the statement of Theorem \ref{theorem: robust} holds with equality.
Therefore, we have that
\begin{equation}
  \mathbb{P}^N\{\{x_i\}_{i=1}^N:~V(n_N^*) \leq \epsilon\} = 1 - \beta,  
\end{equation}
with $\epsilon = 1 - \beta^{\frac{1}{N}}$.


abstract 
% We use the recent develop in non-convex scenario approach to offer a practical convergence guarantee and quantifies the trade-off between the number of iterations and optimization performance, providing stronger assurances than prior work. Numerical examples demonstrate the effectiveness of our approach in providing probabilistic convergence guarantees and evaluating the iteration-performance trade-off.


introduction 
% $\epsilon$ is the expected violation level, while $\hat{\epsilon}$ is the empirical violation level. $\epsilon_a$ represents the expected violation level when $a$ empirical scenarios has been violated, $\delta$ represents the confidence level. 

The authors of \cite{sambharya_data-driven_2024} introduced a data-driven approach, which relies on sample convergence bounds \cite{Langford2001NotBT, JMLR:v6:langford05a}. Their approach evaluates instances of parametric optimization problems using a dataset sampled from the distribution of problem parameters. This method provides probabilistic performance guarantees over different iterations, ensuring that for each evaluated iteration count, the guarantee holds with a user-defined confidence level of \(1 - \beta\). Additionally, they quantified the trade-off between optimization performance and iteration count, with a confidence level of \mbox{\(1 - N^{\rm iter}\beta\)}, where \(N^{\rm iter}\) represents the number of iteration counts evaluated. However, their approach requires that the iteration numbers at which performance is evaluated remain independent of the sampled instances. Thus, it does not offer a pointwise convergence guarantee—meaning they cannot directly evaluate performance at a critical iteration count without also evaluating other iteration numbers. Doing so would lower the overall confidence level of the guarantee, which becomes significantly impacted when evaluating a large number of different iteration counts.

Inspired by \cite{sambharya_data-driven_2024}, we present a data-driven approach based on scenario optimization \cite{modulating_robustness_2013, GarattiCampi2022, non-convex_scenario_optimization2024, Marco_CDC_2020, kostas_2014} to establish the tightest convergence guarantee with high confidence, ensuring no fewer iterations can guarantee convergence by exploiting the support of parameter $x$. Unlike theoretical and computer-assisted analyses, it refines worst-case bounds by leveraging problem-specific properties. Additionally, it differs from existing data-driven methods by simultaneously \emph{learning} the critical iteration count and providing a \emph{generalization guarantee}.

contributions
\begin{itemize}
\item We formulate the problem of establishing convergence guarantees as a scenario optimization problem, learning the number of iterations for convergence and providing a generalization guarantee using the scenario approach.
\item We model the balance between iteration count and optimization performance as a relaxed scenario optimization problem, leveraging recent advancements in the scenario approach to provide data-driven guarantees.
\item We formulate the analysis of determining the upper bound for a user-defined evaluation metric as a scenario optimization problem, offering a generalization guarantee through the scenario approach.
\item We demonstrate the effectiveness of our method with an MPC example, showcasing its ability to provide probabilistic convergence guarantees and evaluate the iteration-performance trade-off.
\end{itemize}

\textit{Outline:} Section II formulates the convergence guarantee problem as a scenario optimization problem and introduces key preliminary concepts in scenario optimization. We apply the scenario approach to establish a probabilistic convergence guarantee and propose a formulation that quantifies the trade-off between the number of iterations and the probability of convergence. Section III demonstrates how the optimizer's performance guarantee can be interpreted as a scenario optimization problem and examines the trade-off between iteration count and performance. Section IV provides numerical examples to illustrate the effectiveness of our method. Section V concludes the paper. % Version 1

\textit{Outline:} Section II formulates the convergence guarantee problem as a robust scenario optimization problem, and further as a relaxed scenario optimizaton problem, providing data-driven guarantees. Section III formulates the analysis of determining the upper bound for a user-defined evaluation metric as scenario optimization problems, offering a generalization guarantee through the scenario approach. Section IV provides numerical examples to illustrate the effectiveness of our method. Section V concludes the paper. % Version 2

\textit{Notation:} For instance, if \( y \) is the decision variable and the problem involves \( N \) scenarios, then \( y^*_N \) represents the optimal solution, and \( y^k_N \) denotes the value of the decision variable \( y \) after the \( k \)th iteration of the optimizer.

section 2
%In this section, we introduce a method that frames convergence analysis as a scenario optimization problem, enabling a probabilistic convergence guarantee.

% We first formulate the problem of finding the convergence guarantee as a scenario optimization problem and then use the latest developments in scenario approach to provide generalization guarantees for our problem.

\begin{definition}[Non-degeneracy, {\protect{\cite[Definition 3]{GarattiCampi2022}}}] \label{non-degeneracy} 
Optimization problem (1) is called \emph{non-degenerate} if its solution coincides with probability \( 1 \) (with respect to the sample \( (\delta_1, \delta_2, \ldots, \delta_N) \)) with the solution that is obtained after eliminating all the constraints that are not of support.
\end{definition}


Compare with the bound in C20 \cite{campi2008exact}, applicable to convex problem without needing non-degeneracy assumption, the tighter bound \cite{Kostas_2015} in C20 can provide a tighter probabilistic convergence guarantee. However, if we want to extend them to the constraint removal section would require the non-degeneracy assumption and is not applicable to our problem, while equations \eqref{compute_t} and \eqref{compute_epsilon} are applicable to the constraint removal process that we present in the subsection. Thus, for the flow of the paper, we only state equations \eqref{compute_t} and \eqref{compute_epsilon}, but following our problem formulation, formula in \cite{campi2008exact} and \cite{Kostas_2015} can also be used to compute the value of $\epsilon$ and therefore, provide a upper bound for the true violation probability $V(n^*_N)$. Potentially, \cite{Kostas_2015} can provide the tightest bound, as it has proven to be tight for problem with only one decision variable. In section \ref{Numerical examples}, we compute the three different bounds and compare the tightness.

section D

Specifically, it provides a framework to quantify the trade-off between computational time and convergence accuracy, offering insights into how iteration budgets can be adjusted to balance efficiency and performance.

There is an inherent trade-off between $n_a$ and $\epsilon_a$, that is what we aim to learn. 


lemma 2 proof

\(\bar{y}\) ranks better than \(y_N^*\) according to the tie-break rule. It implies \(\bar{y} + \rho \sum_{i=1}^{N} \bar{\xi}_{N+M,i} \leq y^*_N + \rho \sum_{i=1}^{N} \xi_{N,i}^*.\) If this inequality holds strictly, it would lead to a contradiction similar to case (a). On the other hand, if equality holds, \((\bar{y}, \bar{\xi}_{N+M,i}, i = 1, \ldots, N)\) would still be preferred over \((y_N^*, \xi_{N,i}^*, i = 1, \ldots, N)\) in problem \eqref{n_relaxed scenario optimization} because \(\bar{y}\) ranks better than \(y_N^*\). This is again a contradiction.

%% to do
Confirm that it satisfies the assumption of VRC (a priori method, fix the number of violated constraints beforehand) and convex relaxation (a posterior method, count the number of violated constraints after solving the relaxed scenario optimization problem. 



Numerical Examples
We first use this example to illustrate how our framework described in Section \ref{section:robust convergence guarantee} can be used to provide a probabilistic convergence guarantees. Since the problem \eqref{n scenario} is convex, though degenerate, following our problem formulation, we can use equation \eqref{compute_t} and \eqref{compute_epsilon} to compute the value of $\epsilon$ with a pre-defined confidence level $\beta = 10^{-4}$, in addition, as stated in the remarks of Section \ref{section:robust convergence guarantee}, the bounds described in \cite[Theorem 1, 3]{Kostas_2015} are also valid following our framework, thus, we display the guarantee obtained from all three methods in the following table.

We also use the example to illustrate the trade-off between the number of iteration and the probability of violation. This trade-off can provide us useful information in practice for online optimization, where the allowed iteration is smaller than the convergence guarantee, and we have to trade off to find a practically best iteration number with a percentage of allowed discarded samples. The result will be as follows.


bibtex

@article{Uncertain_convex_programs2005,
  title={Uncertain convex programs: randomized solutions and confidence levels},
  author={Calafiore, Giuseppe and Campi, Marco},
  journal={Mathematical Programming},
  volume={102},
  pages={25--46},
  year={2005},
  doi={10.1007/s10107-003-0499-y}
}


section 2 C
We now introduce the following two equations \cite{non-convex_scenario_optimization2024}, where \( t \) is the only unknown variable. These equations will later be used to compute \( \epsilon \) in the PAC statement \eqref{PAC_statement}.  
\begin{equation}\label{compute_t}
\frac{\beta}{N} \sum_{m=s_N^*}^{N-1} \binom{m}{s_N^*} t^{m-s_N^*} - \binom{N}{s_N^*} t^{N-s_N^*} = 0,
\end{equation}
where $\beta$ represents the confidence level, $s_N^*$ denotes the \emph{complexity} of the solution, and $N$ is the number of independent random samples. Equation \eqref{compute_t} has a unique solution \( t \) within the interval \((0, 1)\). The value of \( \epsilon \) is then given by:

experiment section
%
%which computes the expected violation probability $\epsilon$ from the empirical violation probability $\hat{\epsilon}$. 
%

The method outlined in \cite{sambharya_data-driven_2024} estimates the expected violation probability from the empirical violation probability using test set bound \cite{JMLR:v6:langford05a}, which focusing solely on generalization. 
%PJG: There is a "the" or "a" missing before "test set bound"
Conversely, scenario-based methods incorporate both learning and generalization guarantees. 

For the method in \cite{sambharya_data-driven_2024}, the threshold iteration number is predefined by the user and based on independence of the samples, and in this method, 
%PG: Which method is the "this method" being referred to here?
we evaluate each point in the trade-off plot by choosing an iteration number threshold as input, and the method outputs the generalized violation probability given the threshold. 

In our approach we choose a targeted number of violations, then compute an optimal iteration number and generalized violation probability. Our methods construct the trade-off curve from a different perspectives, and depends on the solver choice, our methods requires less calls to gain insight about the curve. For example, if the range of iteration number used to solve the parametric problem is large, the method in \cite{sambharya_data-driven_2024} requires to evaluate lots of iteration number to gain insight about the trade-off relationship as no sample-dependent information can be used to choose the iteration number at which empirical violation probability is evaluated. While our methods could evaluated less frequently to gain this trade-off. The number of evaluations could reduce the confidence of the curve, as the overall confidence of the curve is $1 - N^{eval} \times \beta$, where $N^{eval}$ is the number of times we evaluated.

The blue line shows the trade-off between violation probability $\epsilon$ and iteration number obtained using method described in \cite{sambharya_data-driven_2024}, which provide an upper bound for $V(n_a)$.


